On the Probe Complexity of Local Computation Algorithms

The Local Computation Algorithms (LCA) model is a computational model aimed at problem instances with huge inputs and output. For graph problems, the input graph is accessed using probes: strong probes (SP) specify a vertex $v$ and receive as a reply a list of $v$'s neighbors, and weak probes (WP) specify a vertex $v$ and a port number $i$ and receive as a reply $v$'s $i^{th}$ neighbor. Given a local query (e.g., "is a certain vertex in the vertex cover of the input graph?"), an LCA should compute the corresponding local output (e.g., "yes" or "no") while making only a small number of probes, with the requirement that all local outputs form a single global solution (e.g., a legal vertex cover). We study the probe complexity of LCAs that are required to work on graphs that may have arbitrarily large degrees. In particular, such LCAs are expected to probe the graph a number of times that is significantly smaller than the maximum, average, or even minimum degree. For weak probes, we focus on the weak coloring problem. Among our results we show a separation between weak 3-coloring and weak 2-coloring for deterministic LCAs: $\log^* n + O(1)$ weak probes suffice for weak 3-coloring, but $\Omega\left(\frac{\log n}{\log\log n}\right)$ weak probes are required for weak 2-coloring. For strong probes, we consider randomized LCAs for vertex cover and maximal/maximum matching. Our negative results include showing that there are graphs for which finding a \emph{maximal} matching requires $\Omega(\sqrt{n})$ strong probes. On the positive side, we design a randomized LCA that finds a $(1-\epsilon)$ approximation to \emph{maximum} matching in regular graphs, and uses $\frac{1}{\epsilon }^{O\left( \frac{1}{\epsilon ^2}\right)}$ probes, independently of the number of vertices and of their degrees.

==> weak2rand.tex <==
\subsection{Randomized Weak $2$-Coloring LCA}

Let $G=(V,E)$ be a graph, and let $c>0$ be a constant. We assume w.l.o.g. that $G$ is connected. % We say a vertex is \emph{fine} if it has a neighbor with a  different color.

The (global) algorithm is  given as Algorithm~\ref{alg:lca2rand}. \snote{It is also commented out below is a less formal description}
\ignog{

\begin{enumerate}
	\item Every vertex $v$ chooses a rank $r(v) \in [0,1]$ uniformly at random, and (independently) a color $c(v) \in \{0,1\}$ uniformly at random.
	
	\item Every vertex that has a neighbor with a different color fixes its color and becomes a (primary) root.
	\item Every non-root vertex $v$, that is its own grandparent, and whose parent is also a non-root, becomes a secondary root.
	\item Every vertex that is not a  root  (neither primary nor secondary) sets its color to be the opposite color than its parent, recursively.
\end{enumerate}
}

\vspace{10pt}
\begin{algorithm}[H]
	\caption{\textsc{Randomized Weak $2$-coloring LCA}}\label{alg:lca2rand}
	%\DontPrintSemicolon
	\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}\SetKwInOut{Inquiry}{Inquiry}
	
	\Input{$G=(V,E)$, query $v$}
	\Output{$0/1$}
	\BlankLine
	$Roots = \emptyset$\;
	\tcc{Step $1$}
	\ForEach{vertex $v \in V$}{ Sample $color(v) \leftarrow  \{0,1\}$ uniformly at random\;
		Sample $\parent(v) \leftarrow N(v)$ uniformly at random\; }
	\tcc{Step $2$}
	\ForEach{vertex $v \in V$}{\If{$\exists u \in N(v)$ s.t. $color(u) \neq color(v)$}{$Roots \leftarrow v$\;}} 
	\tcc{Step $3$}
	\ForEach{vertex $v \in V$}{\If{$v \notin Roots \wedge \parent(v) \notin Roots \wedge v=\parent(\parent(v))$} {$Roots \leftarrow v$\;}}
		\tcc{Step $4$}
	Return $\textsc{Recursive Color}(G,Roots,v)$\;
\end{algorithm}

\begin{algorithm}[H]
	\caption{\textsc{Recursive Color}}\label{alg:rec}
	%\DontPrintSemicolon
	\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}\SetKwInOut{Inquiry}{Inquiry}
	
	\Input{$G=(V,E)$, $Roots \subseteq V$, query $v$ }
	\Output{$0/1$}
	\BlankLine
	\If{$v \in Roots$}{Return $color(v)$\;}
	\Else{Return $(1-\textsc{Recursive Color}(G, Roots, \parent(v)))$\;}
\end{algorithm}


	\vspace{10pt}
	We need to show that the output of Algorithm~\ref{alg:lca2rand} is a legal  weak $2$-coloring, and 	that it is simulable as an LCA using $O(\log^2{n})$ probes:
	\begin{obs}
		The coloring decreed by Algorithm~\ref{alg:lca2rand} is a legal weak $2$-coloring.
		\end{obs}
		
	\begin{proof}Each vertex that is made a root in Step $2$ necessarily has a neighbor of a different color. The rest of the vertices necessarily have a different color than their parents' (this guarantees a legal coloring as all vertices have parents).
		\end{proof}
	
	\begin{claim}
		Simulating Algorithm~\ref{alg:lca2rand} as an LCA requires $O(\log^2{n})$ w.h.p.
	\end{claim}
	

\begin{proof}
	Let $c>0$ be a constant. For every vertex $v \in V$, if $deg(v) \geq c \log{n}$, we say that $v$'s degree is \emph{high}; otherwise $v$'s degree is \emph{low}. Let $v$ be a high degree vertex. The probability that $v$ does not become a root at Step $2$ is at most $$\left( \frac{1}{2}\right)^{deg(v)} \leq \left( \frac{1}{2}\right)^{c\log{n}}= \frac{1}{n^{c}}.$$ 
	Hence by the union bound, the probability that there exists some high-degree vertex that is not a root after Step $2$ is at most $\frac{1}{n^{c-1}}.$
	
	Henceforth, we  condition on all high degree vertices being roots after Step $2$.% We assume that no low degree vertices are primary roots, as if they ar
	
	Let us now consider a low-degree vertex $v$. The probability that $v$ is a made root at Step $3$ is  at least  $$\frac{1}{deg(\parent(v))} \geq \frac{1}{c\log{n}}.$$
	
	Starting at an arbitrary vertex $u$, we would like to bound the probability that $u$ generates many recursive calls to \textsc{Recursive Color}. Assuming none of the parents of the vertices that participate in these recursive calls is a high-degree vertex, the probability that the  number of recursive calls generated by $u$ is at least  $i$ is at most \snote{we need to be a little careful about the conditioning here, but I think it's basically fine}
	
	\begin{align*}
	   \left( 1-\frac{1}{c\log{n}}\right)^i \leq \frac{1}{n^{c}},
	\end{align*}
	for $i \geq c^2\log^2{n}$ \snote{(or so)}.
	Taking a union bound over all starting vertices completes the proof.
\end{proof}
	

